Fantastic Data and How to Query Them

It is commonly acknowledged that the availability of the huge amount of (training) data is one of the most important factors for many recent advances in Artificial Intelligence (AI). However, datasets are often designed for specific tasks in narrow AI sub areas and there is no unified way to manage and access them. This not only creates unnecessary overheads when training or deploying Machine Learning models but also limits the understanding of the data, which is very important for data-centric AI. In this paper, we present our vision about a unified framework for different datasets so that they can be integrated and queried easily, e.g., using standard query languages. We demonstrate this in our ongoing work to create a framework for datasets in Computer Vision and show its advantages in different scenarios. Our demonstration is available at https://vision.semkg.org.

==> 02-casestd.tex <==
\section{A Case Study of Dynamic Data Acquisition with Vision KG (Anh, 1 page)}

%\begin{itemize}
%\item Example of how to model/present CV datasets using RDF
%\end{itemize}


To realise the ideas outlined above, we carry out a case study by building a unified knowledge graph, namely VisionKG, for CV datasets (e.g, COCO, KITTI or Visual Genome). VisionKG is an Resource Description Framework (RDF) knowledge graph~\citep{Hogan:2021} that contains RDF statements~\citep{Manola:2004} describing the metadata of the images and their visual annotations.

Figure~\ref{fig:vision_kg} illustrates the process of creating VisionKG. 
We first collect CV datasets and analyse visual features from the images and their annotation labels~\textcircled{\raisebox{-0.9pt}{1}}.
To create a unified data model for the annotation labels and visual features, we follow the Linked Data principles~\citep{Bizer:2011} and using RDF data model.
The data entities (e.g, images, boxes, labels) are named using Uniform Resource Identifiers (URI). 
% RDF data model allows the data to be expressed in the form of  \emph{triples} of the form  
% Each statement is given as a triple consisting of a subject, a predicate, and an object.
RDF data model allows the data to be expressed using   \emph{triples} of the form $\mi{\tuple{subject,predicate, object}}$.
For example, to describe ``an image contains a bounding box for a person", we first assign unique URIs, e.g. $\mi{vision.semkg.org/img01}$ and $\mi{vision.semkg.org/box01}$, for the image and the bounding box, respectively; for simplicity, in the remaining text, we skip the prefix. We then utilize existing predicates ($\mi{hasBox, hasObject, rdf:type}$) and class ($\mi{Person}$) in existing knowledge bases to create the following triples for such image:
$\mi{\tuple{img01, hasBox, box01}, \tuple{box01, hasObject, obj01}, \tuple{obj01,rdf:type,Person}}$. 
% state that  e.g. IMGURI01, link the URI denoting the image to the URI denoting box with an RDF predicate \textit{:hasBox}.
%
%\textbf{@Anh: would it make sense to have an example of an image and the corresponding triples here?}
%

Furthermore, we add metadata and semantic annotations for the images, e.g., where the images come from or what are the relations of the boxes in an images (Figure~\ref{fig:vision_kg}~\textcircled{\raisebox{-1pt}{2}}).
To add taxonomy for the labels defined by the original sources, we also link them to WordNet~\footnote{\url{https://wordnet.princeton.edu/}} and Wikidata\footnote{\url{https://www.wikidata.org/}} which are open knowledge graphs. We utilise a semantic reasoner to expand the taxonomy by materialising the labels in each dataset. For example, a box that is labelled as \textit{a pedestrian} is also annotated as \textit{a person} or \textit{a human} (Figure~\ref{fig:vision_kg}~\textcircled{\raisebox{-1pt}{3}}). Hence, our knowledge graph can interlink the annotation labels across label spaces under shared semantic understanding.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=1.0\textwidth]{visionkg.jpg}
    \caption{The overview of VisionKG}
    \label{fig:vision_kg}
\end{figure}

%We use RDF data model to describe the semantic annotations and provide a query interface with SPARQL.

In our case study with VisionKG, we can enable a more convenient way to organise training data and to enable a more robust way to analyse and test trained DNNs.
Using RDF data model to describe the visual annotation labels allows VisionKG to be retrieved using rich semantic query language such as SPARQL~\footnote{\url{https://www.w3.org/TR/rdf-sparql-query/}}. 
The SPARQL query language provides users the ability to describe the query using 
RDF statements which are similar to natural language sentences.
%RDF statements, conjunctions, disjunctions, and optional statements.
For example, Figure 1~\textcircled{\raisebox{-0.9pt}{a}} shows an example of querying \emph{"the images that contain a person holding a cat"}, or Figure 1~\textcircled{\raisebox{-0.9pt}{b}} illustrates a complex query in plain English as \emph{"searche for the trained models to detect \textit{Car} on images of \textit{Car} in crowded traffic scenes or in mountain areas"}. The examplar queries in SPARQL syntaxes can be found in \url{https://vision.semkg.org}.

With VisionKG, users can  organise training data by writing a SPARQL to retrieve the images and labels as desired. This can include an advanced setting like merging training data with the same label from different datasets. Furthermore, users can also get the mixed dataset for validating purposes. Similar to the use case for training data, this includes the case where test data with the same labels are combined from different datasets. In advanced settings, users can test different models with specific labels in one specific dataset or over different datasets. This feature is particularly useful in the case that developers want to target specific applications.



Furthermore, VisionKG can reduce the lack of interoperability, which leads to complex queries that cover all possible cases to unify the labels across different datasets.  For instance, the annotation labels are available in heterogeneous formats and are not consistent across datasets. For example, the {pedestrian} in KITTI dataset~\citep{Geiger:2013} or the {man} in Visual Genome dataset~\citep{Krishna:2017}) are annotated as {person} in COCO dataset. 

\textbf{TODO: explain more.}

Using a semantic resoner, we can expand the taxonomy by materialising the labels in each dataset using the ontology hierarchy, e.g., {pedestrian} or {man} is {SubClassOf} {person}. That means the labels pedestrian or man can be queried as person in case mixing the images from COCO, KITTI and Visual Genome datasets.




